Secure Traffic Lights: Replay Attack Detection for Model-based Smart Traffic Controllers

Rapid urbanization calls for smart traffic management solutions that incorporate sensors, distributed traffic controllers and V2X communication technologies to provide fine-grained traffic control to mitigate congestion. As in many other cyber-physical systems, smart traffic management systems typically lack security measures. This allows numerous opportunities for adversarial entities to craft attacks on the sensor networks, wireless data sharing and/or the distributed traffic controllers. We show that such vulnerabilities can be exploited to disrupt mobility in a large urban area and cause unsafe conditions for drivers and the pedestrians on the roads. Specifically, in this paper, we look into vulnerabilities in model-based traffic controllers and show that, even with state-of-the-art attack detectors in place, false-data injection can be used to hamper mobility. We demonstrate a replay attack by modeling an isolated intersection in VISSIM, a popular traffic simulator and also discuss countermeasures to thwart such attacks.

==> table1.tex <==
% 
\begin{table*}[!h]
\centering
\caption{Percentage of accuracy in guessing the correct key per S-box.}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
\hline
\textbf{attack model}               & \textbf{\#traces} & \textbf{S1} & \textbf{S2} & \textbf{S3} & \textbf{S4} & \textbf{S5} & \textbf{S6} & \textbf{S7} & \textbf{S8}\\ \hline
\multirow{3}{*}{\textbf{baseline}}  & 1000              &  65.38           & 71.79            & 57.69             & 71.79            & 58.97            & 66.66            &  0          &  55.12            \\ \cline{2-10} 
                                    & 1250              &  86.66          & 93.33            & 91.66            & 85            & 73.33             & 80            & 0.0            & 66.66            \\ \cline{2-10} 
                                    & 1500              &  75           & 100            &   75          &   75          & 75            &  75           &   0          &  65           \\ \hline
\multirow{3}{*}{\textbf{variation}} & 1000              & 60.0            & 80.0           & 62.0            &58.0             &56.0             &68.0             &0             &60.0             \\ \cline{2-10} 
                                    & 1250              & 80            &   88          & 88            &  76           & 68            & 92            & 0            &  72           \\ \cline{2-10} 
                                    & 1500              & 95.23             & 100            & 92.85            &  88.09           & 73.80            &  85.71           & 0            & 76.19            \\ \hline
\end{tabular}

\label{tab:tab1}
\end{table*}



% Please add the following required packages to your document preamble:
% 


%% correct guess out of 78: 51    56    45    56    46    52     0    43
%% guess accuracy 65.3846   71.7949   57.6923   71.7949   58.9744   66.6667         0   55.1282
% with length of 1250 
% for 20 iters 
%80    85    90    90    70    80     0    45
%another 20
%100 95 85 75 70 80 0 65
%another 10
%80 100 100 90 80 10 0 90
% with length of 1500 
% for 50 iters 








%% correct guess out of 50 for variation: 30    40    31    29    28    34     0    30
%% guess accuracy 60.0000   80.0000   62.0000   58.0000   56.0000   68.0000         0   60.0000
%% out of 78 iterations of 999 traces.
%% correct guess: 16    53     8    30    27    20    11    14
% Key16 = [ 1     1     1     1     0     0 ;
%           0     0     1     0     1     1 ;
%           1     1     1     0     0     0 ;
%           1     0     1     1     1     0 ;
%           0     1     0     1     1     0 ;
%           1     1     0     0     1     0 ;
%           0     1     0     1     0     0 ;
%           1     0     1     1     0     0 ];
%1500
%95.2381  100.0000   92.8571   88.0952   73.8095   85.7143         0   76.1905
